A Nonparametric Bayesian Framework for Uncertainty Quantification in Stochastic Simulation

When we use simulation to assess the performance of stochastic systems, the input models used to drive simulation experiments are often estimated from finite real-world data. There exist both input model and simulation estimation uncertainties in the system performance estimates. Without strong prior information on the input models and the system mean response surface, in this paper, we propose a Bayesian nonparametric framework to quantify the impact from both sources of uncertainty. Specifically, since the real-world data often represent the variability caused by various latent sources of uncertainty, Dirichlet Processes Mixtures (DPM) based nonparametric input models are introduced to model a mixture of heterogeneous distributions, which can faithfully capture the important features of real-world data, such as multi-modality and skewness. Bayesian posteriors of flexible input models characterize the input model estimation uncertainty, which automatically accounts for both model selection and parameter value uncertainty. Then, input model estimation uncertainty is propagated to outputs by using direct simulation. Thus, under very general conditions, our framework delivers an empirical credible interval accounting for both input and simulation uncertainties. A variance decomposition is further developed to quantify the relative contributions from both sources of uncertainty. Our approach is supported by rigorous theoretical and empirical study.

==> latexmacro.tex <==

%% LaTeX2e file `latexmacro.tex'
%% generated by the `filecontents' environment
%% from source `Gkmn51' on 2001/03/06.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  This macro contains definitions of new \LaTeX commands  %%
%%  that are frequently used by Barry L. Nelson.  This is   %%
%%  a new release of the 'latexmacro.tex' file that I have  %%
%%  distributed for some time.  This release                %%
%%  is designed to be compatible with previous releases,    %%
%%  except for eliminating the \smallheads command.         %%
%%                                                          %%
%%  This releases fixes a few bugs (please report any you   %%
%%  find to nelsonb@random.eng.ohio-state.edu), includes    %%
%%  more documentation, and completes the definitions of    %%
%%  bold-face mathematics characters.                       %%
%%                                                          %%
%%  release 2.01   1/2/92                                   %%
%%  unreleased update 6/9/92  6/22/92 1/19/93 2/3/93        %%
%%                    6/2/93  8/15/93 11/11/93 11/23/93     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% USING THE MACRO:
%% If you name this file latexmacro.tex, then use the following
%% statement just after the \documentstyle{} command:
%%
%%    \input [path] latexmacro
%%
%% LINE SPACING:
%% Define single, one and a half, and double space commands; these
%% may be used anywhere after \begin{document}
%%
\def\double{\par\baselineskip=24pt}
\def\single{\par\baselineskip=12pt}
\def\oneandahalf{\par\baselineskip=18pt}
%%
%% TEXT DIMENSIONS
%% Define text widths \standard, \proceedings and \myletter.
%% \proceedings prints a single, narrow column near the edge of the page.
%% Use these before \begin{document} command.
%%
\def\standard{\oddsidemargin=0in
              \evensidemargin=0in
              \topmargin =-.5in
              \textheight=8.5in
              \textwidth=6.5in}
\def\proceedings{\oddsidemargin=-.5in
                 \evensidemargin=-.5in
                 \textwidth=4.56in
                 \parindent=0.3in
                 \topmargin=-1in
                 \textheight=10in
                 \pagestyle{empty}}
\def\myletter{\oddsidemargin=.3in
                 \evensidemargin=.3in
                 \baselineskip=16pt
                 \textwidth=5.5in
                 \pagestyle{empty}}
%%
%% Define command to pull in letterhead file.
%% This command is specific to VAX/VMS and Arbortext dvips program.
%% Insert your own path.
%%
\def\letterhead{\special{ps: plotfile [is.nelson.com]letterhead.tex 
local}}
%%
%%
%% LISTS:
%% Define \plainlist environment
%%
\newenvironment{plainlist}
{\begin{list}%
{}{\setlength{\leftmargin}{\rightmargin}\setlength{\labelwidth}{0in}}}%
{\end{list}}
%%
%% Define \hangref environment for hanging indentation
%%
\newenvironment{hangref}{\begin{list}{}{\setlength{\itemsep}{0pt}%
\setlength{\parsep}{0pt}\setlength{\leftmargin}{+\parindent}%
\setlength{\itemindent}{-\parindent}}}{\end{list}}
%%
%%
%%
%%
%% MATHEMATICS:
%%Special math symbols
%%
%% operators
\def\E{{\rm E}}
\def\Var{{\rm Var}}
\def\Cov{{\rm Cov}}
\def\Corr{{\rm Corr}}
\def\Bias{{\rm Bias}}
\def\MSE{{\rm MSE}}
\def\CP{{\rm CP}}
\def\trace{{\rm trace}}
\def\tr{{\rm tr}}
%%
%% bold face roman
\def\bA{{\bf A}}
\def\ba{{\bf a}}
\def\bB{{\bf B}}
\def\bb{{\bf b}}
\def\bC{{\bf C}}
\def\bc{{\bf c}}
\def\bD{{\bf D}}
\def\bd{{\bf d}}
\def\bE{{\bf E}}
\def\be{{\bf e}}
\def\bF{{\bf F}}
\def\boldf{{\bf f}}
\def\bG{{\bf G}}
\def\bg{{\bf g}}
\def\bH{{\bf H}}
\def\bh{{\bf h}}
%\def\bi{{\bf i}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bj{{\bf j}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
\def\bL{{\bf L}}
\def\bl{{\bf l}}
\def\bM{{\bf M}}
\def\bm{{\bf m}}
\def\bN{{\bf N}}
\def\bn{{\bf n}}
\def\bO{{\bf O}}
\def\bo{{\bf o}}
\def\bP{{\bf P}}
\def\bp{{\bf p}}
\def\bQ{{\bf Q}}
\def\bq{{\bf q}}
\def\bR{{\bf R}}
\def\br{{\bf r}}
\def\bS{{\bf S}}
\def\bs{{\bf s}}
\def\bT{{\bf T}}
\def\bt{{\bf t}}
\def\bU{{\bf U}}
\def\bu{{\bf u}}
\def\bV{{\bf V}}
\def\bv{{\bf v}}
\def\bW{{\bf W}}
\def\bw{{\bf w}}
\def\bX{{\bf X}}
\def\bx{{\bf x}}
\def\bY{{\bf Y}}
\def\by{{\bf y}}
\def\bZ{{\bf Z}}
\def\bz{{\bf z}}
%%
%% bold face Greek (incomplete)
\def\balpha{\mbox{\boldmath $\alpha$}}
\def\bbeta{\mbox{\boldmath $\beta$}}
\def\bepsilon{\mbox{\boldmath $\epsilon$}}
\def\bvarepsilon{\mbox{\boldmath $\varepsilon$}}
\def\bDelta{{\bf \Delta}}
\def\bdelta{\mbox{\boldmath $\delta$}}
\def\boldeta{\mbox{\boldmath $\eta$}}
\def\bGamma{{\bf \Gamma}}
\def\bgamma{\mbox{\boldmath $\gamma$}}
\def\bLambda{{\bf \Lambda}}
\def\blambda{\mbox{\boldmath $\lambda$}}
\def\bmu{\mbox{\boldmath $\mu$}}
\def\bOmega{{\bf \Omega}}
\def\bpi{\mbox{\boldmath $\pi$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bPsi{{\bf \Psi}}
\def\bpsi{\mbox{\boldmath $\psi$}}
\def\bSigma{{\bf \Sigma}}
\def\bsigma{\mbox{\boldmath $\sigma$}}
\def\bTheta{{\bf \Theta}}
\def\btheta{\mbox{\boldmath $\theta$}}
\def\bXi{{\bf \Xi}}
\def\bxi{\mbox{\boldmath $\xi$}}
%%
%% misc. Greek with hats
\def\betahat{\hat \beta}
\def\bbetahat{\hat{\mbox{\boldmath $\beta$}}}
\def\bdeltahat{\hat{\mbox{\boldmath $\delta$}}}
\def\etahat{\hat{\eta}}
\def\epsilonhat{\hat{\epsilon}}
\def\bepsilonhat{\hat{\mbox{\boldmath $\epsilon$}}}
\def\bgammahat{\hat{\mbox{\boldmath $\gamma$}}}
\def\bmuhat{\hat{\mbox{\boldmath $\mu$}}}
\def\thetahat{\hat \theta}
%%
%% caligraphy letters
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cI{{\cal I}}
\def\cM{{\cal M}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cY{{\cal Y}}
%%
%% tt letters
\def\tS{{\tt S}}
\def\tC{{\tt C}}
\def\tI{{\tt I}}
\def\tT{{\tt T}}
%%
%% vec notation
\def\vp{\vec{p}}
\def\bvP{\vec{{\bf P}}}
%%
%% bold face numbers
\def\b1{{\bf 1}}
\def\bzero{{\bf 0}}
%%
%% \blot gives a square at end of formulas and proofs
%% (thanks to Marc Posner)
\def\blot{\quad {$\vcenter{\vbox{\hrule height.4pt
             \hbox{\vrule width.4pt height.9ex \kern.9ex \vrule 
width.4pt}
             \hrule height.4pt}}$}}
%%



\newcommand{\JH}[1]{\textcolor{red}{#1}}




%% End of latexmacro
